Multi-Source Data Fusion for Cyberattack Detection in Power Systems

Cyberattacks can cause a severe impact on power systems unless detected early. However, accurate and timely detection in critical infrastructure systems presents challenges, e.g., due to zero-day vulnerability exploitations and the cyber-physical nature of the system coupled with the need for high reliability and resilience of the physical system. Conventional rule-based and anomaly-based intrusion detection system (IDS) tools are insufficient for detecting zero-day cyber intrusions in the industrial control system (ICS) networks. Hence, in this work, we show that fusing information from multiple data sources can help identify cyber-induced incidents and reduce false positives. Specifically, we present how to recognize and address the barriers that can prevent the accurate use of multiple data sources for fusion-based detection. We perform multi-source data fusion for training IDS in a cyber-physical power system testbed where we collect cyber and physical side data from multiple sensors emulating real-world data sources that would be found in a utility and synthesizes these into features for algorithms to detect intrusions. Results are presented using the proposed data fusion application to infer False Data and Command injection-based Man-in- The-Middle (MiTM) attacks. Post collection, the data fusion application uses time-synchronized merge and extracts features followed by pre-processing such as imputation and encoding before training supervised, semi-supervised, and unsupervised learning models to evaluate the performance of the IDS. A major finding is the improvement of detection accuracy by fusion of features from cyber, security, and physical domains. Additionally, we observed the co-training technique performs at par with supervised learning methods when fed with our features.

==> Content/9_challenges.tex <==
\section{Discussion}\label{challenges}
\textcolor{red}{temp; MOVE TO FUTURE WORK: Knowledge extraction prior to fusion is currently not incorporated in this work but can be easily leveraged since we perform sequential merge of features.}

\textcolor{red}{temp; MOVE TO discussion: Supervised, semi-supervised, and un-supervised techniques all need to be explored since each can be more appropriate in different scenarios.  
%
Other work fails to consider packet header details in creating feature space.  Our previous work \cite{} included evaluation of cyber-side features like retransmission, round trip time (RTT), and flow counts; this motivates the need of extraction of measurements from packet capture. 
Deploying the data to a datasource such as Elasticsearch makes data aggregation, filtering, visualization convenient.  
}


\textcolor{red}{temp;Move to DISCUSSION ?:
A challenge with power system data fusion is the location of the fusion engine. If the fusion and inference engine are located outside the control network, security to pull out the data is an issue. In the real world, it is important to consider how the physical data will be available to a fusion engine, the size of the database, and whether anonymization techniques may be applied to preserve privacy.   If such challenges are overcome, multi-sensor fusion enable stakeholders to classify data to identify and localize mis-operations due to system faults as well as intruder-instigated failure.}


\textcolor{red}{[like in paper 1, you don't really need a future work section in a journal paper, but a discussion section (or could be a final subsection of previous section) instead, so I suggest turning this section into that instead, but of course keeping our list of next-steps for ourselves. Discussing the "current challenges" in the discussion section is still a good idea and it can also still mention next steps/future work, but you really want to capture/highlight the main aspects and key results of the paper in this discussion section.  You could check different papers to get examples of how this might be done well. There are likely a variety of different good ways. ]} Data Fusion is a prior step followed before
state estimation. Hence, in our current work we have used fusion to infer an attack
and the time when the attack was performed. In our future work we will explore, if
such inference can improve the cyber physical state estimation. Also in the current
work, we are using decimal to compress the information of the binary array, which is
only efficient in storage and neither interpretable nor comparable. Our next step is
coming up with a method to better map a variant-length of data (BI, BO, AI, AO) to a
fixed-dimension space where the mapped data will have the following properties,
which enable us to easily find anomaly event chronologically and spatially:
\begin{enumerate}
    \item Reconstructed data will be the same if their original data are the same
    \item Reconstructed data will be close if their original data are similar
    \item Reconstructed data will be an outlier if the original data has values that is out of
normal range
\end{enumerate}
